What Knowledge Gets Distilled in Knowledge Distillation?

Knowledge distillation aims to transfer useful information from a teacher network to a student network, with the primary goal of improving the student's performance for the task at hand. Over the years, there has a been a deluge of novel techniques and use cases of knowledge distillation. Yet, despite the various improvements, there seems to be a glaring gap in the community's fundamental understanding of the process. Specifically, what is the knowledge that gets distilled in knowledge distillation? In other words, in what ways does the student become similar to the teacher? Does it start to localize objects in the same way? Does it get fooled by the same adversarial samples? Does its data invariance properties become similar? Our work presents a comprehensive study to try to answer these questions. We show that existing methods can indeed indirectly distill these properties beyond improving task performance. We further study why knowledge distillation might work this way, and show that our findings have practical implications as well.

==> experiments_new.tex <==
\vspace{-5pt}
\section{Experiments}\label{sec:exp}
\vspace{-5pt}

%\yh{Overall, I think it is better to includes the following two more studies (see the two scenarios in the intro): a model trained with softlabel (not from teacher), and it is not more similar to the teacher; a model distilled from one teacher, but top1 acc is not improved, but still similar to teacher in some ways. Maybe we can figure out that in which studies we can include these two cases.}
% use the image classification task as our case study, and
%In our analyses,
We now discuss our experimental design. 
%We  use ImageNet \cite{imagenet}, MNIST \cite{lecun-mnist1998}, as well as images from artistic domains \cite{geirhos2021partial}. 
%Unless otherwise mentioned, for all the analyses, the distillation procedure is performed using the training dataset, and evaluation is performed on the corresponding validation dataset. 
To reach conclusions that are generalizable across different architectures and datasets, and robust across independent runs, we experiment with a variety of teacher-student architectures, and tune the hyperparameters so that the distillation objective improves the test performance of the student compared to independent training.  For each setting, we average the results over two independent runs. 
%each time, the distilled student and independent student (without distillation) are trained using the same random seed. 
We report the top-1 accuracy of all the models in the appendix. The notation $\texttt{Net}_1 \rightarrow \texttt{Net}_2$ indicates distilling the knowledge of $\texttt{Net}_1$ (teacher) into $\texttt{Net}_2$ (student). 
%The network architectures for the teacher and the student are different for different analysis, and the reason for those choices are given in those respective sections. 

%As mentioned before, we are more interested in studying knowledge transfer between the teacher and the student in ways other than top-1 accuracy. Hence, the main text doesn't discuss the top-1 accuracy obtained either by the teacher or the student. For reference, those results can be found in the supplementary. In general, we do try to find the best configuration of hyper-parameters so that the resulting distilled student improves in accuracy over the independent student. 

\vspace{-2pt}

\vspace{-2pt}
\subsection{Does adversarial vulnerability get distilled?}\label{sec:adv}
\vspace{2pt}
%\as{Adversarially Robust Networks has technically done this before/}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1\textwidth]{figs/adv_results.png}
    \vspace{-15pt}
    \caption{The images which fool the teacher fool the distilled student more than the independent student in \textbf{(a)}, \textbf{(b)} and \textbf{(d)}, but not in \textbf{(e)}. If the adversarial attack is generated using a foreign network (ResNet18, \textbf{(c)}), it fails to convincingly fool the distilled student more than the independent one. 
    %\textbf{(a, b} and \textbf{d)} 
    %\yh{I have a general concern for our plotting, in many cases, we actually want to make difference more obvious by only plot in certain scales, such as (a) (b). But this will make all difference more obvious than before. For example, in (d), at the first glimpse it seems hint improves a lot, but actually it is not true, only if we check numbers. So maybe for later case, we do not plot but rather just report numbers?} 
    }
    \label{fig:adv}
    \vspace{-5pt}
\end{figure*}

Next, we study the transfer of a different kind of property. If we design an adversarial image to fool the teacher, then will that same image fool the distilled student more than the independent student?
% Two different neural networks (teacher and independent student) will have their own separate ways of either correctly or incorrectly classifying an image. Now, in the previous section, we saw that the interpretability of the distilled students can become similar to that of the teacher when classifying correctly. Could this mean that the student \emph{misclassifies} in similar ways as the teacher as well? 
%\yh{I think for the previous section, we study how do networks make predication based on the regions they focus on, but this does not mean what is currently written, which read sounds like we do the following experiment: only for images correctly classified by all teacher, ind and distilled, sim(teacher, distilled) > sim(teacher, ind). Actually, I think maybe we can do the following study, for those images misclassfied by ind, but correctly classified by distilled and tea, to compare their grad-cam, to see if the difference it even bigger.}


\textbf{Experimental setup:} We train a teacher, a distilled student, and an independent student for ImageNet classification. Given 5000 random test images, we convert each image $I$ into an adversarial image $I^{adv}$ using iterative FGSM \cite{fgsm, iter-fgsm} (see appendix for details), whose goal is to fool the teacher, so that teacher's prediction for $I^{adv}$ changes from its original prediction for $I$. Fooling rate is then defined as the fraction of adversarial images which succeed at this task. In our experiments, we use only this fraction of adversarial images which fool the teacher, and apply them to different students.  
%We create the adversarial images using iterative FGSM \cite{fgsm, iter-fgsm}; please see the supplementary for details of creating the images.% understand the process of
% First, we pass the clean image through the target network (to be fooled). Then we compute the gradient of the loss function with respect to the image ($\nabla_X$), and then update the image in the \emph{opposite} way, so as to maximize the loss ($J(X, y_{true})$). The update is bounded to be within a range [$X - \epsilon, X + \epsilon$], so that the change in the image is imperceptible. This whole process constitutes one step of FGSM, and the iterative version of this method does this for $k$ steps ($k=5$ in our case). The process can be depicted formally through Eq.~\ref{eq:fgsm}, where $\alpha$ controls the step size:
% \begin{align}
%     X^{adv}_{0} = X, \quad 
%     X^{adv}_{t+1} = Clip_{X, \epsilon}\bigl\{ X^{adv}_{t} + \alpha \sign \bigl( \nabla_X J(X^{adv}_{N}, y_{true})  \bigr) \bigr\} 
% \label{eq:fgsm}
% \end{align}
%We report results for ImageNet dataset. 
%We take 5000 randomly sampled test images from the validation set, and convert them to their adversarial forms, so that the teacher network makes mistakes while classifying them. 

% \yh{Although it is easy to understand what does fooling rate mean, do we need to explicitly mention how do we calculate them? Also I think we should study deeper in this analysis beyond only using fooling rate. For example, let's say we have ten images (0-9). images 0-7 can fool the teacher, image 0 can fool independent student (rate=0.1) , but images 8,9 can fool the distilled student (rate=0.2). The fooling rate is doubled, but its behavior is less similar to the teacher} 

%%We start with ResNet50 $\rightarrow$ ResNet18 as the setting. 

% The adversarial attack is successful in ~85\% of the cases (among 5000 test images) for all the teachers. Fig.~\ref{fig:adv} shows the fooling rate (y-axis) when applying these successful adversarial images that fooled the teacher to different types of students (x-axis).

\textbf{Results:} We evaluate four configurations: (i) ResNet50 $\rightarrow$ ResNet18, (ii) VGG19 $\rightarrow$ VGG11, (iii) VGG19 $\rightarrow$ ResNet18, (iv) ViT (ViT-b-32) \cite{vit}  $\rightarrow$ ResNet18. 
%The attack is successful in $\sim$85\% of the cases for all the teachers. 
The fooling rate is $\sim$85\% for all the teachers.
Fig.~\ref{fig:adv} shows the fooling rate (y-axis) when applying these successful adversarial images to different types of students (x-axis).
We see that for ResNet50 $\rightarrow$ ResNet18, the ability to fool the independent student drops to 44.2\%, which is expected since the adversarial images aren't designed for that student.  In distilled students, we see an increase in the fooling rate relative to the independent one across all distillation methods (48\%-52\%). The trend holds for VGG19 $\rightarrow$ VGG11 and VGG19 $\rightarrow$ ResNet18; 
Fig.~\ref{fig:adv} (b, d). When distillation is done from a transformer to a CNN (ViT $\rightarrow$ ResNet18) the fooling rates remain similar for the independent and distilled students; Fig.~\ref{fig:adv} (e). Here, we don't see the student becoming similar to the teacher to the extent observed for a CNN $\rightarrow$ CNN distillation.

%, especially if it was generated through multiple rounds of targeted attack
%The fooling method that we choose, i

\textbf{Discussion:} This result is surprising. Iterative FGSM is a white box attack, which means that it has full access to the target model (teacher), including its weights and gradients. Thus, the adversarial examples are specifically crafted to fool the teacher. In contrast, the student never has direct access to the weights and gradients of the teacher, regardless of the distillation method. Yet, by simply trying to mimic the teacher's soft probabilities ($KL$) or an intermediate feature layer
\yj{($Hint$, $CRD$)}, the student network inherits, to some extent, the particular way that a teacher is fooled. 

% But, does this happen only because the distillation process improves the student's accuracy? To test this hypothesis, we performed $VGG19 \rightarrow VGG11$ distillation using $KL$ and $Hint$ using different hyper-parameter values ($\alpha, \beta, \gamma$ in Eq.~\ref{eq:kl}, ~\ref{eq:hint}), and chose the distilled students that are no more accurate than the independent student. The top-1 accuracy of the models are: (i) $S_{Ind}$: 68.89\%, (ii) $S_{KL}$: 68.48\% and (iii) $S_{Hint}$: 67.94\%. Fig.~\ref{fig:adv} (e) shows the results of attacking these students using successful adversarial images crafted for VGG19. Interestingly, the fooling rates for the distilled students are still higher compared to the independent student. We tie this result to the question raised in the beginning: even if distillation does not improve the accuracy, as was shown in \cite{cho-iccv2019}, the distillation procedure could still be transferring some other form of knowledge into the student.  

%However, we want to make sure that the
We conduct an additional study to ensure that the reason the distilled student is getting fooled more is because it is being attacked specifically by its \emph{teacher's} adversarial images; i.e., if those images are designed for some other network, would the difference in fooling rates still be high?
%We perform an additional experiment to rule out a different conclusion.  Specifically, it may be that the distillation process itself makes the student more vulnerable to \emph{any} adversarial image, and not necessarily to those designed specifically for the teacher. 
We test this in the VGG19 $\rightarrow$ VGG11 setting. This time we generate adversarial images ($I \rightarrow I^{adv}$) to fool an ImageNet pre-trained ResNet18 network, instead of VGG19 (the teacher).  We then use those images to attack the same VGG11 students from the VGG19 $\rightarrow$ VGG11 setting.  In Fig.~\ref{fig:adv} (c), we see that the fooling rates for the independent and distilled students remain similar. This indicates that distillation itself does not make the student more vulnerable to \emph{any} adversarial attack, and instead, an increase in fooling rate can be attributed to the student's inheritance of the teacher's adversarial vulnerability. 


%; i.e., there is no significant increase in fooling rate for the distilled students

%However, there could be a different conclusion drawn from this result. It is possible that the distillation process makes the student vulnerable to \emph{any} adversarial image, and not necessarily to those designed for the teacher. 

%\subsection{Does knowledge about invariance to change get distilled?}
\vspace{-2pt}
\subsection{Does invariance to data transformations get distilled?}\label{sec:inv}
\vspace{-2pt}

We have studied whether the response properties on single images get transferred from the teacher to the student. Now suppose that the teacher is invariant to certain changes in data, either learned explicitly through data augmentation or implicitly due to architectural choices. Can such properties about \emph{changes in images} get transferred during distillation? 
%have its own biases or 
%In other words, if the teacher was more invariant to a particular change, and the student less so, will it become more invariant to that change after distillation? 
%All the experiments that follow will have this theme: we create two versions of a test image, $X_1$ and $X_2$, which are different random variations of a particular change. For example, $X_1$ and $X_2$ could be the same image augmented to have different hue levels. We pass both images through a network \ut{either teacher or student} and report how frequently their predicted classes match. We call this the agreement score, which we compute over the 50k images of the ImageNet validation set.

%\subsubsection{Color invariance}\label{sec:color_inv}

\textbf{Experimental setup:} We study color invariance as a transferable property. 
%(The appendix (C.4) contains a similar experiment where we study invariance to random shifts in images instead and find a similar result).
We train three models for ImageNet classification: a teacher, a distilled and an independent student. While training the teacher, we add color jitter in addition to the standard augmentations (random crops, horizontal flips). Specifically, we alter an image's brightness, contrast, saturation, and hue, with magnitudes sampled uniformly in [0, 0.4] for the first three, and in [0, 0.2] for hue. This way, the teacher gets to see the same image with different color properties during training and can become color invariant. When training the student, we only use the standard augmentations \emph{without} color jittering, and see whether such a distilled student can indirectly inherit the color invariance property through the teacher. 
%And if the student does become invariant to color changes, then it should produce the same classification label for two different color augmentations of the same image. 
%In contrast, an independent student is less likely to become color invariant, since it never learned about it explicitly.
%inherit that property and 

\textbf{Results:} We start with the ResNet50 $\rightarrow$ ResNet18 configuration. After training, we evaluate the models on 50k ImageNet validation images. For each image $X$, we construct its augmented version $X'$ by altering the color properties in the same way as done while training the teacher. Fig.~\ref{fig:color} (a) depicts the agreement scores between $X$ and $X'$ (y-axis) for different models (x-axis). The teacher (T), being trained to have that property, achieves a high score of 92.5\%. The independent student, which is not trained to be color invariant, has a much lower score of 71.3\%. But, when the color-invariant teacher is used to perform distillation using $KL$ or $CRD$, the agreement scores of the students jump up to 82.1\% and 79.5\% respectively. To ensure that this increase is not due to some regularizing property of the distillation methods that has nothing to do with the teacher, we repeat the experiment, this time with a ResNet50 teacher (T$^{*}$) that is not trained with color augmentation. The new agreement scores for the distilled students (marked by *; e.g., KL$^{*}$) drop considerably compared to the previous case. This is a strong indication that the student does inherit \emph{teacher-specific} invariance properties during distillation. 

\begin{figure*}[t]
    \centering
    \includegraphics[width=1\textwidth]{figs/inv_results.png}
    \vspace{-15pt}
    \caption{\textbf{(a)} Agreement between two images  with different color properties. * indicates distillation done by a teacher T$^{*}$ not trained to be color invariant. \textbf{(b, c)} Agreement between two images having increasingly different color properties. \textbf{(d)} Effect of different layers used in $Hint$ distillation.}
    \label{fig:color}
    \vspace{-5pt}
\end{figure*}


In Fig.~\ref{fig:color}(b), we show that this trend in agreement scores (y-axis) holds even when the magnitude of change in brightness, contrast and saturation (x-axis) is increased to create $X'$ from $X$. We repeat this experiment for Swin-tiny (a transformer) \cite{swin} $\rightarrow$ ResNet18 in Fig.~\ref{fig:color}(c). We again see some improvements in the agreement scores of the distilled students. This increase, however, is not as significant as that observed in the previous CNN $\rightarrow$ CNN setting. Throughout this work, we find that distilling the properties from a transformer teacher into a CNN student is difficult. The implicit biases introduced due to architectural differences between the teacher (transformer) and student (CNN) seem too big, as was studied in \cite{cnn-vs-vit}, to be overcome by current distillation methods.

We also note the ineffectiveness of $Hint$ in distilling this knowledge. Our guess for this is the choice of $l$ for distillation, which is typically set to be in the middle of the network as opposed to deeper layers where $KL$ and $CRD$ operate.
%Our initial guess for this is because the default $Hint$ asks the student to mimic the teacher at somewhere in the middle of the network. This is different than $KL$ and $CRD$, which operate at deeper levels of the network. 
So, we perform an ablation study for $Hint$, where the student mimics a different feature of the teacher each time; starting from a coarse feature of resolution $56 \times 56$ (F1) to the output scores (logits) of the teacher network (F7). We plot the agreement scores in Fig.~\ref{fig:color}(d), where we see that the score increases as we choose deeper features. Mimicking the deeper layers likely constrains the overall student more compared to a middle layer, since in the latter case, the rest of the student (beyond middle layer) could still function differently compared to the teacher.
%However, why should the information about color invariance be better encoded in deeper rather than shallower layers is an open question.



\textbf{Discussion:} In sum, color invariance can be transferred during distillation. This is quite surprising since the teacher is not used in a way which would expose any of its invariance properties to the student. Remember that all the student has to do during distillation is to match the teacher's features for an image $X$; i.e., the student does not get to see its color augmented version, $X'$, during training. If so, then why should it get to know how the teacher would have responded to $X'$? 
%We try providing an answer in Sec.~\ref{sec:why}.  

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=1\textwidth]{figs/crop.pdf}
%     \vspace{-5pt}
%     \caption{Crop invariance}
%     \label{fig:color}
% \end{figure*}


% \subsubsection{Shift invariance}
% The $X_1$ and $X_2$ discussed in the previous section could have different aspect ratios. However, shift invariance is a more subtle property
\vspace{-2pt}
\subsection{Does knowledge about unseen domains get distilled?}\label{sec:ood}
\vspace{-2pt}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=1\textwidth]{figs/ood_agreement.png}
    \vspace{-15pt}
    \caption{\textbf{Left:} Does knowledge transferred about one domain give knowledge about other unseen domains? \textbf{Right:} Consensus scores between teacher and student for images from unseen domains.}
    \label{fig:ood}
    \vspace{-5pt}
\end{figure*}

So far, our analysis has revolved around the original ImageNet dataset, something that was used to perform the distillation itself. So, does the teacher only transfer its knowledge pertaining to this domain, or also of domains it has never seen (Fig.~\ref{fig:ood} left)? 

\textbf{Experimental setup:} To test this, we first perform distillation using two settings (i) VGG19 $\rightarrow$ ResNet18 and (ii) Swin-Base \cite{swin} $\rightarrow$ Swin-Tiny, where the training of the teacher, as well as distillation is done on ImageNet. During test time, we take an image from an unseen domain and see how frequently the student's and teacher's class predictions match for it (regardless of whether the predicted label is correct or incorrect), which we call the consensus score.
% Note that this agreement score is different than the one used in Sec.~\ref{sec:inv}. 
%During the distillation process, the essential goal is to make the student mimic the teacher on some dataset of interest. Does this make the student more similar to the teacher on some other domains as well, which was not used for training? 
%Note that the goal is not to report the accuracy of either the teacher or the student for this new domain, but rather to see if their behaviour is similar, even if it is incorrect. 
For the unseen domains, we consider the five datasets proposed in \cite{geirhos2021partial}: $\texttt{sketch}$, $\texttt{stylized}$, $\texttt{edge}$, $\texttt{silhouette}$, $\texttt{cue conflict}$. Images from these domains are originally from ImageNet, but have had their properties modified. 
%E.g., $\texttt{sketch}$ contains ImageNet images converted to their sketch form, $\texttt{stylized}$ contains images which have their content preserved, but with different style. 

%\yh{I think we need to define "agreement" here, since this "agreement" is different from the previous one. Also, I still think we need to have more settings, which at least has a transformer one. Since the current transferring results are not that conclusive if we see the resnet case}
\textbf{Results:} Fig.~\ref{fig:ood} (right) shows the consensus scores between the teacher and the student (y-axis). We see a nearly consistent increase in consensus brought about by the distillation methods in both settings. The extent of this increase, however, differs among the domains. There are cases, for example, in VGG19 $\rightarrow$ ResNet18, where consensus over images from $\texttt{edge}$ domain increases over 100\% (12\% $\rightarrow$  $\ge$30\%) by some distillation methods. On the other hand, the increase can also be relatively modest in certain cases: e.g. Swin-Base $\rightarrow$ Swin-Tiny in $\texttt{stylized}$ domain. 
%Now, from Sec.~\ref{sec:ref}, remember that 


\textbf{Discussion:} \cite{stanton-neurips2021} showed that the agreement in classification between the teacher and distilled student is not much different than that to an independent student on CIFAR. We find this to be true in our ImageNet classification experiments as well. That is why the increase in agreement observed for unseen domains is surprising. After all, if the agreement is not increasing when images are from the seen domain, why should it increase when they are from an unseen domain?  It is possible that there is more scope for increase in agreement in unseen domains vs seen domain. The consensus score between teacher and independent student for the seen domain is $\ge$75\% (appendix), whereas for an unseen domain, e.g. $\texttt{sketch}$, it is $\le$40\%. So, it might not be that knowledge distillation does not work, as the authors wondered in \cite{stanton-neurips2021}, but its effect could be more prominent in certain situations.     

%These results might seem in contradiction to that presented in \cite{stanton-neurips2021}, where the authors studied agreement on the validation set of ImageNet itself (not an unseen domain), and found no significant improvement by the distilled student compared to an independent student. 
%Again, we believe that this is not a trivial result: it is not clear if matching the output spaces of two complex neural networks

\subsection{Does localization knowledge get distilled?}
\vspace{-2pt}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1\textwidth]{figs/cam.png}
    \vspace{-13pt}
    \caption{\textbf{Left:} An example of how the distilled student can focus on similar regions as the teacher while classifying an image. \textbf{Right:} \% where teacher's CAM is more similar to the distilled student's CAM than to the independent student's CAM. The red line indicates chance performance (50\%).}%color indicates the corresponding student's score. 
    \label{fig:cam}
    \vspace{-5pt}
\end{figure*}
%where 50\% (chance performance) lies
%\yh{Overall, I think we should include one transformer one in this study}

We start by studying whether the localization properties of a teacher transfers to a student through knowledge distillation.  For example, suppose that the teacher classifies an image as a cat by focusing on its face, and an independent student classifies it as a cat by focusing on its fur. After knowledge distillation, will the student focus \emph{more} on the face when classifying the image as a cat?  
%Different neural networks, especially of different architectures, will look at different regions of an image to classify it as one of the classes. Hence, the independent student and the teacher might have different class activation maps (CAMs). But does distillation push the map of the student to be closer to the teacher's? 

%use ImageNet for this experiment.
% (teacher or student)
\textbf{Experimental setup:} We train three models for ImageNet classification: a teacher, a distilled and an independent student. For each network, we obtain the class activation map (CAM) of the ground-truth class for each of random 5000 test images, using Grad-CAM \cite{grad-cam}, which visualizes the pixels that a classifier focuses on for a given class. We then compute how often (in terms of \% of images) the teacher's CAM is more similar (using cosine similarity) to the distilled student's CAM than to the independent student's CAM. A score of $>$50\% means that, on average, the distilled student's CAMs become more similar to those of the teacher than without distillation. As a sanity check, we also compute the same metric between the teacher's CAM and the CAMs of two independent students trained with different seeds (\emph{Ind}), which should be equally distant from the teacher (score of $\sim$50\%).
%$Ind$ computes the same frequency metric between the teacher's CAM and the CAMs of two independent students (both without distillation) trained with two random seeds. This is a sanity check baseline to show that these two models should be equally distant from the teacher, hence achieving a score of $\sim$50\%.  
%We compute this similarity through cosine similarity between the two activation maps. 
%Then, for each distillation method, w
%compares two random seeds of the independently trained student; 

\textbf{Results:} Fig.~\ref{fig:cam} (right) shows the results for two configurations of teacher-student architectures: (i) ResNet50 $\rightarrow$ ResNet18 and (ii) VGG19 $\rightarrow$ VGG11. For \emph{KL} and \emph{CRD}, we observe a significant increase in similarity compared to random chance (as achieved by the \emph{Ind} baseline).  \emph{Hint} also shows a consistent increase, although the magnitude is not as large.  
%We see that the activation maps of the ResNet-18 (student) produced through $KD$ distillation is twice as likely to be more similar to the teacher's, than an independent student's activation map. 

\textbf{Discussion:} This experiment shows that having access to the teacher's class-probabilities, i.e. confidence for the ground-truth class, can give information on where the teacher is focusing on while making the classification decision. This corroborates, to some degree, the result obtained in the Grad-CAM paper \cite{grad-cam}, which showed that if the network is very confident of the presence of an object in an image, it focuses on a particular region (Fig.~1(c) in \cite{grad-cam}), and when it is much less confident, it focuses on some other region (Fig.~7(d) in \cite{grad-cam}). 
%Not all distillation methods are created equal, however, and some have a lesser ability to make the activation map more similar to the teacher (e.g. $Hint$). 
Fig.~\ref{fig:cam} (left) shows a sample test image and the corresponding CAMs produced by the independent student (left), teacher (middle), and distilled student (right) for the ground-truth class. The distilled student looks at similar regions as the teacher, and moves away from the regions it was looking at initially (independent student). 
%Importantly, we are not interested in the correctness of any network's CAM; rather, we are using CAM as a tool to study whether a distilled student's CAMs become similar to those of the teacher's.  And our analysis indicates this to be the case for all three distillation techniques, albeit with varying degrees.  
So, regardless of the correctness of any network's CAM, our analysis shows that a distilled student's CAM does become similar to those of the teacher for all three distillation techniques, albeit with varying degrees.

%we do not wish to convey that the teacher's activation maps are better (though they might be for the task at hand), but rather to study whether the student's maps become similar to its, even if it is not the best map.
% should we talk about why we should study this, considering the reasons mentioned in the original KD paper about the teacher probably knowing more about the soft-classes in the image which the student might not know about, and hence we should test whether that hypothesis is actually happening (DISCUSS)


\vspace{-3pt}
\subsection{Other studies}
\vspace{-3pt}
In appendix, we study additional aspects of a model such as shape/texture bias, invariance to random crops, and find that even these obscure properties can transfer from a teacher to the student. We also explore the following questions: If we can find alternative ways of increasing a student's performance (e.g. using crafted soft labels), will that student gain similar knowledge as a distilled student? If distillation cannot increase the student's performance, is there no knowledge transferred? 

%\yj{We might want to say what other studies we have done, and where to find them in the supp.  This can be just 2-3 lines.  For example, ``We provide more analysis on pseudo-label precision and recall, and results with true out-of-distribution unlabeled data. These can be found in the Appendix.''}


%methods trying to make the student mimic the teacher.
%that we notice throughout this work, 

 
%Note that the dataset used during distillation is the standard ImageNet, so any improvement observed in \ut{Fig. X} is only an indirect result of student mimicking the teacher. 
%We don't see any improvements through $Hint$, however, similar to results shown in Sec.~\ref{sec:inv}.  
\vspace{-2pt}


\vspace{-2pt}
\section{Applications}\label{sec:mnist}
\vspace{-2pt}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1\textwidth]{figs/mnist_results_new.png}
    \vspace{-15pt}
    \caption{\textbf{Left:} The teacher is trained on three domains: $\texttt{MNIST-Orig}$, $\texttt{MNIST-Color}$, and $\texttt{MNIST-M}$. Distillation is done only on $\texttt{MNIST-Orig}$. \textbf{Right:} Test accuracy of the students. Note the increase in performance on $\texttt{MNIST-Color}$ \& $\texttt{MNIST-M}$ domains by the distilled students.}
    \label{fig:mnist}
    \vspace{-5pt}
\end{figure*}

Beyond the exploratory angle of studying whether certain properties get transferred during distillation, the idea of a student becoming similar to a teacher in a broad sense has practical implications. We discuss a good and a bad example in this section.
%Previous sections have had an exploratory angle to them, where we have primarily been interested if certain (often obscure) properties can transfer via the distillation process. Our finding, which is that the student becomes similar to the teacher on a much broader level, can have practical implications. In this section, we present two of those - a good example and a bad example.

%\ut{The previous sections provided a \yj{comprehensive study} of the indirect effects of the distillation process. While we believe that those important properties of a model, and consequently the ability to transfer them, is important in itself, their study also paves the way for two sides of practical applications - \yj{a good example and a bad example.}}
\vspace{-2pt}
\subsection{The Good: the free ability of domain adaptation}\label{sec:good_mnist}
\vspace{-2pt}
Consider the following setup: the teacher is trained for a task by observing data from multiple domains ($\mathcal{D}_1 \cup \mathcal{D}_2$). It is then used to distill knowledge into a student on only $\mathcal{D}_1$. Apart from getting knowledge about $\mathcal{D}_1$, will the student also get knowledge about $\mathcal{D}_2$ indirectly? 

%Consider the following setup: if $\texttt{T}$ is trained on $\mathcal{D}_1 \cup \mathcal{D}_2$, and is used to distill knowledge into student on $\mathcal{D}_1$, does the student's performance increase on $\mathcal{D}_2$ as well?

% Consider the following: a model ($T$) is trained for image classification on a dataset consisting of multiple domains; $\{\mathcal{D}_1 \cup \mathcal{D}_2 ... \cup \mathcal{D}_n\}$. It is then used as a teacher to distill knowledge into a student ($S_d$) on \emph{one} of those domains: $T \rightarrow S_d$ on $D_1$. The independent student ($S$) is also trained on $\mathcal{D}_1$. Will the distilled student perform better than the independent student on the rest of the domains $\mathcal{D}_2, ...\mathcal{D}_n$? 

% as our testbed
\textbf{Experimental setup:} We use MNIST digit recognition, and train the teacher on three domains: (i) $\texttt{MNIST-orig}$: original gray-scale images from MNIST, (ii) $\texttt{MNIST-Color}$: background of each image randomly colored, and (iii) $\texttt{MNIST-M}$ \cite{mnist-m}: MNIST digits pasted on random natural image patches. The student models are trained \emph{only} on $\texttt{MNIST-orig}$ and evaluated (top-1 accuracy) on all three domains. The network architecture is same for both the teacher and the student (see appendix). 

\textbf{Results:} When the independent student is trained only on $\texttt{MNIST-orig}$, its performance drops on the other unseen domains, which is expected due to domain shift. The distilled students, however, are able to significantly improve their performance on both $\texttt{MNIST-Color}$ and $\texttt{MNIST-M}$; see Fig.~\ref{fig:mnist}.

%\yh{For "no color information", Do you mean the input image or the response? If it is the second one, then I feel the claim is a bit strong, since response is a function of both input and the model, which has knowledge about color} 

\textbf{Discussion:} This result shows distillation's practical benefits: once a teacher acquires an ability through computationally intensive training (e.g., training on multiple datasets), that ability can be distilled into a student, to a decent extent, through a much simpler process. The student sees the teacher's response to \emph{gray-scale} images ($\texttt{MNIST-orig}$) that lack any color information. But that information helps the student to deal better with \emph{colored} images (e.g., $\texttt{MNIST-Color}$), likely because the teacher has learned a domain-invariant representation (e.g., shape) which is distilled to the student.

\vspace{-2pt}
\subsection{The Bad: Students can inherit harmful biases from the teacher}\label{sec:bad_bias}
\vspace{-2pt}

Consider the problem of classifying gender from human faces. Imagine an independent student which performs the classification fairly across all races. The teacher, on the other hand, is biased against certain races, but is more accurate than the student \emph{on average}. Will the student, which was originally fair, become unfair after mimicking the unfair teacher?

\textbf{Experimental setup:} We consider a ResNet20 $\rightarrow$ ResNet20 setting, and use FairFace dataset \cite{fairface}, which contains images of human faces from 7 different races with their gender labeled. From its training split, we create two different subsets ($\mathcal{D}_s$ and $\mathcal{D}_t$) with the following objectives - (i) $\mathcal{D}_s$ has a particular racial composition so that a model trained on it will perform fairly across all races during test time; (ii) $\mathcal{D}_t$'s composition is intended to make the model perform unfairly for certain races. The exact composition of $\mathcal{D}_s$ and $\mathcal{D}_t$ is given in the appendix. The teacher is trained on $\mathcal{D}_t$ whereas the independent/distilled students are trained on $\mathcal{D}_s$. We use $KL$ for distillation.

\begin{wrapfigure}[11]{r}{0.5\textwidth}
	\centering
 	\vspace{-13pt}
	%\hspace*{5pt}
	\includegraphics[width=0.5\textwidth]{figs/kd_bias_bad.png}
	\vspace{-5pt}
\end{wrapfigure}
\textbf{Results:} We observe in the figure on the right that the independent student performs roughly fairly across all races, which is what we intended. The teacher is more accurate than the student, but performs relatively poorly on faces from Race 3 compared to others. After distillation, we observe that the student's \emph{overall} accuracy improves, but the gain in accuracy is less for images from Race 3. So, when it is trained on $\mathcal{D}_s$ by itself, it behaves fairly. But when it mimics the teacher on $\mathcal{D}_s$, it becomes unfair.

\textbf{Discussion:} The practical takeaway from the experiment is that knowledge distillation can bring forth behaviour which is considered socially problematic if it is viewed simply as a blackbox tool to increase a student's performance on test data, as it did in the previous example. Proper care must hence be taken regarding the transfer/amplification of unwanted biases in the student.



% \subsection{Key takeaways:}
% Add text later.
